The meaning of a program change is a change to the program's meaning

Programming is the activity of modifying a program in order to bring about specific changes in its behaviour. Yet programming language theory almost exclusively focuses on the meaning of programs. We motivate a "change-oriented" viewpoint from which the meaning of a program change is a change to the program's meaning.

==> experiment/def/fonts.tex <==
% save defaults
\edef\keptrmdefault{\rmdefault}
\edef\keptsfdefault{\sfdefault}
\edef\keptttdefault{\ttdefault}
\usepackage[math]{iwona}
% restore defaults
\edef\rmdefault{\keptrmdefault}
\edef\sfdefault{\keptsfdefault}
\edef\ttdefault{\keptttdefault}

\usepackage[T1]{fontenc}
\usepackage{libertine}
\usepackage[scaled=0.75]{beramono}
\usepackage{upgreek}


==> experiment/def/layout.tex <==
\everymath{\displaystyle}

\allowdisplaybreaks

% I find the align environments use a bit too much vertical spacing.
\addtolength{\jot}{-0.25em}

% XeTeX/LuaTeX-style micro-kerning and whatnot. Stops LaTeX going mad with hyphenation.
\usepackage{microtype}

\raggedbottom % sane vertical paragraph justification

\hypersetup{ % not using recent enough version of hyperref for [hidelinks] option
    colorlinks=false,
    pdfborder={0 0 0},
}

% Put section and chapter numbering in margins, and color red.
\makeatletter
\def\@seccntformat#1{\protect\makebox[0pt][r]{\textcolor{red}{\csname
      the#1\endcsname}\hspace{6pt}}} \makeatother


==> experiment/def/macros.tex <==
\newcommand*{\src}[1]{\mathsf{src}({#1})}
\newcommand*{\tgt}[1]{\mathsf{tgt}({#1})}
\newcommand*{\delt}[1]{\mathbf{#1}}
\newcommand*{\ins}[1]{\greenuline{#1}}
\newcommand*{\del}[1]{\reduline{#1}}
\newcommand*{\change}[1]{\blueuline{#1}}
\newcommand*{\hole}{\scalebox{0.8}{$\medsquare$}}
\newcommand*{\comp}{\mathrel{\Cdot}}

% Terms and delta terms.
\newcommand*{\exApp}[2]{{#1}\,{#2}}
\newcommand*{\exAppDelLeft}[2]{\exApp{\del{#1}}{#2}}
\newcommand*{\exAppDelRight}[2]{\exApp{#1}{\del{#2}}}
\newcommand*{\exAppInsLeft}[2]{\exApp{\ins{#1}}{#2}}
\newcommand*{\exAppInsRight}[2]{\exApp{#1}{\ins{#2}}}
\newcommand*{\exDel}[1]{\del{#1}}
\newcommand*{\exEmpty}{\varepsilon}
\newcommand*{\exIns}[1]{\ins{#1}}
\newcommand*{\exHole}{\hole}
\newcommand*{\exInl}[1]{\kw{inl}\;#1}
\newcommand*{\exInlChange}[1]{\change{\kw{inl}}\;#1}
\newcommand*{\exInlDel}[1]{\del{\kw{inl}}\;#1}
\newcommand*{\exInlIns}[1]{\ins{\kw{inl}}\;#1}
\newcommand*{\exInr}[1]{\kw{inr}\;#1}
\newcommand*{\exInrChange}[1]{\change{\kw{inr}}\;#1}
\newcommand*{\exInrDel}[1]{\del{\kw{inr}}\;#1}
\newcommand*{\exInrIns}[1]{\ins{\kw{inr}}\;#1}
\newcommand*{\exFun}[2]{\lambda{#1}.{#2}}
\newcommand*{\exFunDel}[2]{\del{\lambda{#1}}.{#2}}
\newcommand*{\exFunIns}[2]{\ins{\lambda{#1}}.{#2}}
\newcommand*{\exMatchPair}[4]{\kw{match}\;#1\;\exPair{#2}{#3}.#4}
\newcommand*{\exMatchSum}[5]{\kw{match}\;#1\;\{\exInl{#2}.#3; \exInr{#4}.#5\}}
% Need to escape to text mode or underlining will go awry.
\newcommand*{\exMatchSumDelOne}[5]{\text{\del{$\kw{match}$}$\;#1\;$}\text{\del{$\{\exInl{#2}.#3; \exInr{#4}.#5\}$}}}
\newcommand*{\exMatchSumDelTwo}[5]{\text{\del{$\kw{match}\;#1\;\{\exInl{#2}.$}}#3\text{\del{$; \exInr{#4}.#5\}$}}}
\newcommand*{\exMatchSumDelThree}[5]{\text{\del{$\kw{match}\;#1\;\{\exInl{#2}.#3; \exInr{#4}.$}}#5\text{\del{$\}$}}}
\newcommand*{\exMatchSumInsOne}[5]{\text{\ins{$\kw{match}$}$\;#1\;$}\text{\ins{$\{\exInl{#2}.#3; \exInr{#4}.#5\}$}}}
\newcommand*{\exMatchSumInsTwo}[5]{\text{\ins{$\kw{match}\;#1\;\{\exInl{#2}.$}}#3\text{\ins{$; \exInr{#4}.#5\}$}}}
\newcommand*{\exMatchSumInsThree}[5]{\text{\ins{$\kw{match}\;#1\;\{\exInl{#2}.#3; \exInr{#4}.$}}#5\text{\ins{$\}$}}}
\newcommand*{\exPair}[2]{(#1,#2)}
\newcommand*{\exPairDelLeft}[2]{\del{(#1,\,}#2\del{)}}
\newcommand*{\exPairDelRight}[2]{\del{(}#1\del{,#2)}}
\newcommand*{\exPairInsLeft}[2]{\ins{(#1,\,}#2\ins{)}}
\newcommand*{\exPairInsRight}[2]{\ins{(}#1\ins{,#2)}}
\newcommand*{\exRoll}[1]{\kw{roll}\;#1}
\newcommand*{\exRollChange}[1]{\change{\kw{roll}}\;#1}
\newcommand*{\exRollDel}[1]{\del{\kw{roll}}\;#1}
\newcommand*{\exRollIns}[1]{\ins{\kw{roll}}\;#1}
\newcommand*{\exUnit}{\ast}
\newcommand*{\exUnroll}[1]{\kw{unroll}\;#1}
\newcommand*{\exUnrollChange}[1]{\change{\kw{unroll}}\;#1}
\newcommand*{\exUnrollDel}[1]{\del{\kw{unroll}}\;#1}
\newcommand*{\exUnrollIns}[1]{\ins{\kw{unroll}}\;#1}
\newcommand*{\exVal}[2]{#1_{#2}}
\newcommand*{\exVar}[1]{#1}
\newcommand*{\exVarReplace}[2]{\change{#2}{_{#1}}}

\newcommand*{\plug}[2]{{#1}[#2]}
\newcommand*{\plugIns}[2]{\ins{#1}[#2]}
\newcommand*{\plugDel}[2]{\del{#1}[#2]}

\newcommand*{\tyEmpty}{\varepsilon}
\newcommand*{\tyUnit}{1}
\newcommand*{\tySum}[2]{{#1}+{#2}}
\newcommand*{\tySumInsLeft}[2]{{\ins{#1\;+}}\;{#2}}
\newcommand*{\tySumInsRight}[2]{{#1}\;\ins{+\;{#2}}}
\newcommand*{\tyProd}[2]{{#1}\times{#2}}
\newcommand*{\tyProdInsLeft}[2]{{\ins{#1\;\times}}\;{#2}}
\newcommand*{\tyProdInsRight}[2]{{#1}\;\ins{\times\;{#2}}}
\newcommand*{\tyFun}[2]{{#1}\rightarrow{#2}}
\newcommand*{\tyFunInsLeft}[2]{{\ins{#1\;\rightarrow}}\;{#2}}
\newcommand*{\tyFunInsRight}[2]{{#1}\;\ins{{\rightarrow}\;{#2}}}

\newcommand*{\compat}{\smile}
\newcommand*{\pathTo}{\leftrightsquigarrow}
\newcommand*{\replace}[2]{#1\mathrel{:=:}#2}
\newcommand*{\residual}[2]{{#1}/{#2}}
\newcommand*{\subst}[3]{#1\{{#2}/{#3}\}}
\newcommand*{\substPath}{\rightsquigarrow}
\newcommand*{\eval}{\Rightarrow}

\definecolor{mygreen}{rgb}{0.0, 0.5, 0.0}

% See http://tex.stackexchange.com/questions/325866
\newcommand{\reduline}[1]{{\color{red}\uline{{\color{black}#1}}}}
\newcommand{\greenuline}[1]{{\color{mygreen}\uline{{\color{black}#1}}}}
\newcommand{\blueuline}[1]{{\color{blue}\uline{{\color{black}#1}}}}


==> experiment/def/packages.tex <==
\usepackage{extpfeil}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{float}
\usepackage{stmaryrd}
\usepackage[usenames,dvipsnames]{color}
\usepackage{hyperref}
\usepackage{mathpartir}
\usepackage{microtype}
\usepackage{tikz}
\usepackage{xspace}
\usepackage{calc} % for \widthof
\usepackage{pifont} % \for \ding
\usepackage{listings}
\newcommand\hmmax{0} % see http://tex.stackexchange.com/questions/3676
\newcommand\bmmax{0}
\usepackage{bm}
\usetikzlibrary{automata}
\usetikzlibrary{positioning}
\usepackage{mathtools}
\usepackage{natbib}
\usepackage{cancel}
\usepackage{array}
\usepackage{tikz-cd}
\usepackage{soul}
\usepackage{ulem}

\input{../tex-common/MnSymbol-medsquare}
\input{def/uline}


==> experiment/def/uline.tex <==
% http://tex.stackexchange.com/questions/133243

\makeatletter
\newcommand*{\saved@uline}{}
\let\saved@uline\uline

\newcommand*{\mathuline}{%
  \mathpalette{\math@uline\saved@uline}%
}
\newcommand*{\math@uline}[3]{%
  % #1: ulem command
  % #2: math style
  % #3: contents
  \mbox{#1{$#2#3\m@th$}}%
}

% optional
\renewcommand*{\uline}{%
  \relax
  \ifmmode
    \expandafter\mathuline
  \else
    \expandafter\saved@uline
  \fi
}
\makeatother


==> experiment/fig/compatible.tex <==
\begin{figure}[H]
\noindent \shadebox{$\delt{e} \compat \delt{e}'$}
\begin{smathpar}
  \inferrule*
  {
    \strut
  }
  {
    \exEmpty \compat \delt{e}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
  }
  {
    \plugIns{C}{\delt{e}} \compat \delt{e}'
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
  }
  {
    \plugDel{C}{\delt{e}} \compat \plugDel{C}{\delt{e}'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
  }
  {
    \exInl{\delt{e}} \compat \exInl{\delt{e}'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
  }
  {
    \exInr{\delt{e}} \compat \exInr{\delt{e}'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
    \\
    \delt{e}_1 \compat \delt{e}_1'
    \\
    \delt{e}_2 \compat \delt{e}_2'
  }
  {
    \exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2} \compat \exMatchSum{\delt{e}'}{x}{\delt{e}_1'}{y}{\delt{e}_2'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}_1 \compat \delt{e}_1'
    \\
    \delt{e}_2 \compat \delt{e}_2'
  }
  {
    \exPair{\delt{e}_1}{\delt{e}_2} \compat \exPair{\delt{e}_1'}{\delt{e}_2'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \compat \delt{e}'
  }
  {
    \exFun{x}{\delt{e}} \compat \exFun{x}{\delt{e}'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}_1 \compat \delt{e}_1'
    \\
    \delt{e}_2 \compat \delt{e}_2'
  }
  {
    \exApp{\delt{e}_1}{\delt{e}_2} \compat \exApp{\delt{e}_1'}{\delt{e}_2'}
  }
\end{smathpar}
\caption{Compatibility of coinitial deltas}
\end{figure}


==> experiment/fig/delta-term-equations.tex <==
\begin{figure}[H]
  \begin{align*}
    \exEmpty \comp \delt{e}
    & \simeq
    \delt{e}
    \\
    \delt{e} \comp \exEmpty
    & \simeq
    \delt{e}
    \\
    \plugIns{C}{\delt{e}} \comp \plugDel{C}{\delt{e}'}
    & \simeq
    \delt{e} \comp \delt{e}'
    \\
    \plugIns{C}{\delt{e}} \comp \plug{C}{\delt{e}'}
    & \simeq
    \plugIns{C}{\delt{e} \comp \delt{e}'}
    \\
    \plug{C}{\delt{e}} \comp \plugDel{C}{\delt{e}'}
    & \simeq
    \plugDel{C}{\delt{e} \comp \delt{e}'}
    \\
    \exInlChange{\delt{e}} \comp \exInrChange{\delt{e}'}
    & \simeq
    \delt{e} \comp \delt{e}'
    \\
    \exInrChange{\delt{e}} \comp \exInlChange{\delt{e}'}
    & \simeq
    \delt{e} \comp \delt{e}'
  \end{align*}
\caption{Equational theory of deltas}
\end{figure}


==> experiment/fig/delta-term.tex <==
\begin{figure}[H]
\begin{syntaxfig}
\mbox{Term delta}
&
\delt{e}
&
::=
&
\sub{\exEmpty}{e}
\mid
\plugIns{C}{\delt{e}}
\mid
\plugDel{C}{\delt{e}}
\mid
\exInl{\delt{e}}
\mid
\exInlChange{\delt{e}}
\mid
\exInr{\delt{e}}
\mid
\exInrChange{\delt{e}}
\mid
\\
&&&
\exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2}
\mid
\exPair{\delt{e}}{\delt{e'}}
\mid
\exFun{x}{\delt{e}}
\mid
\exApp{\delt{e}}{\delt{e}}
\\[2mm]
\mbox{Term context}
&
C
&
::=
&
\hole
\mid
\exInl{C}
\mid
\exInr{C}
\mid
\\
&&&
\exMatchSum{C}{x}{e}{y}{e'}
\mid
\\
&&&
\exMatchSum{e}{x}{C}{y}{e'}
\mid
\\
&&&
\exMatchSum{e}{x}{e'}{y}{C}
\mid
\exPair{C}{e}
\mid
\exPair{e}{C}
\mid
\\
&&&
\exFun{x}{C}
\mid
\exApp{C}{e}
\mid
\exApp{e}{C}
\end{syntaxfig}
\\[2mm]
\noindent \shadebox{$\delt{e}: e \pathTo e'$}
\begin{smathpar}
  \inferrule*
  {
    \strut
  }
  {
    \sub{\exEmpty}{e}: e \pathTo e
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \plugIns{C}{\delt{e}}: e \pathTo C[e']
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \plugDel{C}{\delt{e}}: C[e] \pathTo e'
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \exInlChange{\delt{e}}: \exInr{e} \pathTo \exInl{e'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \exInrChange{\delt{e}}: \exInl{e} \pathTo \exInr{e'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \exInl{\delt{e}}: \exInl{e} \pathTo \exInl{e'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \exInr{\delt{e}}: \exInr{e} \pathTo \exInr{e'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
    \\
    \delt{e}_1: e_1 \pathTo e_1'
    \\
    \delt{e}_2: e_2 \pathTo e_2'
  }
  {
    \exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2}: \\
    \exMatchSum{e}{x}{e_1}{y}{e_2} \pathTo \exMatchSum{e'}{x}{e_1'}{y}{e_2'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}: e \pathTo e'
  }
  {
    \exFun{x}{\delt{e}}: \exFun{x}{e} \pathTo \exFun{x}{e'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}_1: e_1 \pathTo e_1'
    \\
    \delt{e}_2: e_2 \pathTo e_2'
  }
  {
    \exApp{\delt{e}_1}{\delt{e}_2}: \exApp{e_1}{e_2} \pathTo \exApp{e_1'}{e_2'}
  }
\end{smathpar}
\caption{Delta terms}
\end{figure}


==> experiment/fig/residual/delta-after-delta.tex <==
\begin{figure}[H]
  \noindent \shadebox{$\residual{\delt{e}}{\delt{e}'}$}
{\small
  \begin{align*}
    \residual{\exEmpty}{\delt{e}}
    &=
    \exEmpty
    \\
    \residual{\delt{e}}{\exEmpty}
    &=
    \delt{e}
    \\
    \residual{(\exFun{x}{\delt{e}})}{\exFun{x}{\delt{e}'}}
    &=
    \exFun{x}{\residual{\delt{e}}{\delt{e}'}}
    \\
    \residual{(\exFunIns{x}{\delt{e}})}{\delt{e}'}
    &=
    \exFunIns{x}{\residual{\delt{e}}{\delt{e}'}}
    \\
    \residual{\delt{e}}{\exFunIns{x}{\delt{e}'}}
    &=
    \exFun{x}{\residual{\delt{e}}{\delt{e}'}}
    \\
    \residual{(\exApp{\delt{e}_1}{\delt{e}_2})}{(\exApp{\delt{e}_1'}{\delt{e}_2'})}
    &=
    \exApp{\residual{\delt{e}_1}{\delt{e}_1'}}{\residual{\delt{e}_2}{\delt{e}_2'}}
    \\
    \residual{(\exAppInsLeft{e}{\delt{e}})}{\delt{e}'}
    &=
    \exAppInsLeft{e}{\residual{\delt{e}}{\delt{e}'}}
    \\
    \residual{\delt{e}}{(\exAppInsLeft{e}{\delt{e}'})}
    &=
    \exApp{\exEmpty}{\residual{\delt{e}}{\delt{e}'}}
    \\
    \residual{(\exAppInsRight{\delt{e}}{e})}{\delt{e}'}
    &=
    \exAppInsRight{\residual{\delt{e}}{\delt{e}'}}{e}
    \\
    \residual{\delt{e}}{(\exAppInsRight{\delt{e}'}{e})}
    &=
    \exApp{\residual{\delt{e}}{\delt{e}'}}{\exEmpty}
  \end{align*}
}
\caption{Residual of $\delt{e}$ after compatible $\delt{e}'$}
\end{figure}


==> experiment/fig/residual/delta-after-eval.tex <==
\begin{figure}[H]
\noindent \shadebox{$\delt{e} \eval \delt{v}$}
\begin{smathpar}
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exInl{\delt{e}} \eval \exInl{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exInlChange{\delt{e}} \eval \exInlChange{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exInlIns{\delt{e}} \eval \exInlIns{\delt{v}}
  }
  %
  \and
  %
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exInlDel{\delt{e}} \eval \exInlDel{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \exInl{\delt{v}}
    \\
    \subst{\delt{e}_1}{\delt{v}}{x} \eval \delt{v}'
  }
  {
    \exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2} \eval \delt{v}'
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo v'$}]
  {
    \delt{e} \eval \exInlChange{\delt{v}}
    \\
    \subst{e_1}{v}{x} \eval v''
  }
  {
    \exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2} \eval \change{v''}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: \exInl{v} \pathTo v'$}]
  {
    \delt{e} \eval \exInlIns{\delt{v}}
    \\
    \subst{\delt{e}_1}{\delt{v}}{x} \eval v''
  }
  {
    \exMatchSum{\delt{e}}{x}{\delt{e}_1}{y}{\delt{e}_2} \eval \change{v''}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo \exInl{v'}$}]
  {
    \delt{e} \eval \delt{v}
    \\
    \subst{e_1}{v'}{x} \eval v''
  }
  {
    \exMatchSumInsOne{\delt{e}}{x}{e_1}{y}{e_2} \eval \change{v''}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo v'$}]
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exMatchSumDelOne{\delt{e}}{x}{e_1}{y}{e_2} \eval \change{v'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e}_1 \eval \delt{v}_1
    \\
    \delt{e}_2 \eval \delt{v}_2
  }
  {
    \exPair{\delt{e}_1}{\delt{e}_2} \eval \exPair{\delt{v}_1}{\delt{v}_2}
  }
  %
  \and
  %
  \inferrule*
  {
    e \eval v
    \\
    \delt{e} \eval \delt{v}
  }
  {
    \exPairInsLeft{e}{\delt{e}} \eval \exPairInsLeft{v}{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
    \\
    e \eval v
  }
  {
    \exPairInsRight{\delt{e}}{e} \eval \exPairInsRight{\delt{v}}{v}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \exFun{x}{\delt{e}''}
    \\
    \delt{e}' \eval \delt{v}
    \\
    \subst{\delt{e}''}{\delt{v}}{x} \eval \delt{v}'
  }
  {
    \exApp{\delt{e}}{\delt{e}'} \eval \delt{v}'
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo v'$}]
  {
    e \eval \exFun{x}{e'}
    \\
    \delt{e} \eval \delt{v}
    \\
    \subst{e'}{v'}{x} \eval v''
  }
  {
    \exAppInsLeft{e}{\delt{e}} \eval \change{v''}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo \exFun{x}{e'}$}]
  {
    \delt{e} \eval \delt{v}
    \\
    e \eval v'
    \\
    \subst{e'}{v'}{x} \eval v''
  }
  {
    \exAppInsRight{\delt{e}}{e} \eval \change{v''}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo v'$}]
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exAppDelLeft{e}{\delt{e}} \eval \change{v'}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo v'$}]
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exAppDelRight{\delt{e}}{e} \eval \change{v'}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exRoll{\delt{e}} \eval \exRoll{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exRollIns{\delt{e}} \eval \exRollIns{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exRollDel{\delt{e}} \eval \exRollDel{\delt{v}}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \exRoll{\delt{v}}
  }
  {
    \exUnroll{\delt{e}} \eval \delt{v}
  }
  %
  \and
  %
  \inferrule*[right={$\delt{v}: v \pathTo \exRoll{v'}$}]
  {
    \delt{e} \eval \delt{v}
  }
  {
    \exUnrollIns{\delt{e}} \eval \delt{v} \comp \exRollDel{\exEmpty}
  }
  %
  \and
  %
  \inferrule*
  {
    \delt{e} \eval \exRollDel{\delt{v}}
  }
  {
    \exUnrollDel{\delt{e}} \eval \delt{v}
  }
\end{smathpar}
\caption{Delta evaluation}
\end{figure}


==> experiment/fig/residual/illustrate/substitution.tex <==
\begin{nscenter}
\scalebox{0.8}{
\begin{tikzpicture}[node distance=1.5cm, auto]
  \node (P) [node distance=2cm] {
    $(e,v)$
  };
  \node (R) [left of=P, below of=P] {
    $\subst{e}{v}{x}$
  };
  \node (RPrime) [below of=P, right of=P] {
    $(e',v')$
  };
  \node (PPrime) [right of=R, below of=R] {
    $\subst{e'}{v'}{x}$
  };
  \draw[->] (P) to node [swap] {$\subst{\param}{\param}{x}$} (R);
  \draw[->] (P) to node {$(\delt{e},\delt{v})$} (RPrime);
  \draw[dotted,->] (R) to node [swap] {$\subst{\delt{e}}{\delt{v}}{x}$} (PPrime);
  \draw[->] (RPrime) to node {$\subst{\param}{\param}{x}$} (PPrime);
\end{tikzpicture}
}
\end{nscenter}


==> experiment/fig/substitution.tex <==
\begin{figure}[H]
\noindent \shadebox{$\subst{\delt{e}}{\delt{v}}{x}$, where $\delt{v}: v \pathTo v'$}
{\small\begin{align*}
\subst{\sub{\exEmpty}{x}}{\delt{v}}{x}
&=
\sub{\delt{v}}{x}
\\
\subst{\exVarReplace{x}{y}}{\delt{v}}{x}
&=
\exVal{\del{v}}{\change{y}}
\\
\subst{\exVarReplace{y}{x}}{\delt{v}}{x}
&=
\exVal{\ins{v'}}{\change{x}}
\\
\subst{\sub{\exEmpty}{(\exInl{e})}}{\delt{v}}{x}
&=
\exInl{\subst{\sub{\exEmpty}{e}}{\delt{v}}{x}}
\\
\subst{(\exInl{\delt{e}})}{\delt{v}}{x}
&=
\exInl{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{(\exInlIns{\delt{e}})}{\delt{v}}{x}
&=
\exInlIns{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{(\exInlDel{\delt{e}})}{\delt{v}}{x}
&=
\exInlDel{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{(\exInlChange{\delt{e}})}{\delt{v}}{x}
&=
\exInlChange{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{\sub{\exEmpty}{\exPair{e}{e'}}}{\delt{v}}{x}
&=
\exPair{\subst{\sub{\exEmpty}{e}}{\delt{v}}{x}}{\subst{\sub{\exEmpty}{e'}}{\delt{v}}{x}}
\\
\subst{\exPair{\delt{e}}{\delt{e'}}}{\delt{v}}{x}
&=
\exPair{\subst{\delt{e}}{\delt{v}}{x}}{\subst{\delt{e'}}{\delt{v}}{x}}
\\
\subst{\exPairInsLeft{e}{\delt{e}}}{\delt{v}}{x}
&=
\exPairInsLeft{\subst{e}{v'}{x}}{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{\exPairInsRight{\delt{e}}{e}}{\delt{v}}{x}
&=
\exPairInsRight{\subst{\delt{e}}{\delt{v}}{x}}{\subst{e}{v'}{x}}
\\
\subst{\exPairDelLeft{e}{\delt{e}}}{\delt{v}}{x}
&=
\exPairDelLeft{\subst{e}{v}{x}}{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{\exPairDelRight{\delt{e}}{e}}{\delt{v}}{x}
&=
\exPairDelRight{\subst{\delt{e}}{\delt{v}}{x}}{\subst{e}{v}{x}}
\\
\subst{(\exFunIns{x}{\delt{e}})}{\delt{v}}{x}
&=
\exFunIns{x}{\subst{\delt{e}}{\del{v}}{x}}
\\
\subst{(\exFunIns{y}{\delt{e}})}{\delt{v}}{x}
&=
\exFunIns{y}{\subst{\delt{e}}{\delt{v}}{x}}
& (y \neq x)
\\
\subst{(\exFunDel{x}{\delt{e}})}{\delt{v}}{x}
&=
\exFunDel{x}{\subst{\delt{e}}{\ins{v'}}{x}}
\\
\subst{(\exFunDel{y}{\delt{e}})}{\delt{v}}{x}
&=
\exFunDel{y}{\subst{\delt{e}}{\delt{v}}{x}}
&
(y \neq x)
\\
\subst{\sub{\exEmpty}{(\exApp{e}{e'})}}{\delt{v}}{x}
&=
\exApp{\subst{\sub{\exEmpty}{e}}{\delt{v}}{x}}{\subst{\sub{\exEmpty}{e'}}{\delt{v}}{x}}
\\
\subst{(\exApp{\delt{e}}{\delt{e'}})}{\delt{v}}{x}
&=
\exApp{\subst{\delt{e}}{\delt{v}}{x}}{\subst{\delt{e'}}{\delt{v}}{x}}
\\
\subst{(\exAppInsLeft{e}{\delt{e}})}{\delt{v}}{x}
&=
\exAppInsLeft{\subst{e}{v'}{x}}{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{(\exAppInsRight{\delt{e}}{e})}{\delt{v}}{x}
&=
\exAppInsRight{\subst{\delt{e}}{\delt{v}}{x}}{\subst{e}{v'}{x}}
\\
\subst{(\exAppDelLeft{e}{\delt{e}})}{\delt{v}}{x}
&=
\exAppDelLeft{\subst{e}{v}{x}}{\subst{\delt{e}}{\delt{v}}{x}}
\\
\subst{(\exAppDelRight{\delt{e}}{e})}{\delt{v}}{x}
&=
\exAppDelRight{\subst{\delt{e}}{\delt{v}}{x}}{\subst{e}{v}{x}}
\end{align*}}
\caption{Delta-substitution}
\end{figure}


==> experiment/fig/term.tex <==
\begin{figure}[H]
\begin{syntaxfig}
\mbox{Term}
&
e
&
::=
&
\exHole
\mid
\exVar{x}
\mid
\exUnit
\mid
\exInl{e}
\mid
\exInr{e}
\mid
\exMatchSum{e}{x}{e}{x}{e}
\mid
\\
&&&
\exPair{e}{e}
\mid
\exMatchPair{e}{x}{x}{e}
\mid
\exFun{x}{e}
\mid
\exApp{e}{e}
\end{syntaxfig}
\caption{Terms}
\end{figure}


==> experiment/fig/value.tex <==
\begin{figure}[H]
\begin{syntaxfig}
\mbox{Value}
&
v
&
::=
&
\exInl{v}
\mid
\exInr{v}
\mid
\exPair{v_1}{v_2}
\mid
\exFun{x}{e}
\end{syntaxfig}
\\[1mm]
\caption{Values}
\end{figure}


==> experiment/sec/evaluation.tex <==
\section{Evaluation}

\input{fig/value}
\input{fig/substitution}
\input{fig/residual/illustrate/substitution}
\input{fig/residual/delta-after-eval}


==> experiment/sec/related-work.tex <==
\section{Related work}

\paragraph{Patch theory.}

\cite{angiuli14}

\paragraph{Static differentiation.}

\cite{cai14}

\paragraph{Formalising editing.}

\cite{amsden14,edwards06}


==> experiment/sec/syntax.tex <==
\section{Syntax}

\input{fig/term}
\input{fig/delta-term}
\input{fig/delta-term-equations}
\input{fig/compatible}
\input{fig/residual/delta-after-delta}


==> tex-common/MnSymbol-asterisk.tex <==
% Bring in asterisk symbols from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\Mnthinstar}{\mathrel}{MnSyC}{134}
\DeclareMathSymbol{\Mnast}{\mathrel}{MnSyC}{135}


==> tex-common/MnSymbol-bowtie.tex <==
\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\let\bowtie\relax
\DeclareMathSymbol{\bowtie}{\mathrel}{MnSyC}{38}


==> tex-common/MnSymbol-cong.tex <==
% Bring in \cong from MnSymbol.

\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareMathSymbol{\Cong}{\mathrel}{MnSyD}{12}


==> tex-common/MnSymbol-inequalities.tex <==
\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\sqcupdot}{\mathrel}{MnSyC}{68}
\DeclareMathSymbol{\sqcapdot}{\mathrel}{MnSyC}{69}
\DeclareMathSymbol{\eqslantgtr}{\mathrel}{MnSyC}{228}
\DeclareMathSymbol{\eqslantless}{\mathrel}{MnSyC}{227}

\DeclareMathSymbol{\less}{\mathrel}{MnSyD}{64}
\DeclareMathSymbol{\gtr}{\mathrel}{MnSyD}{65}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\sqlt}{\mathrel}{MnSyD}{88}
\DeclareMathSymbol{\sqgt}{\mathrel}{MnSyD}{89}
\DeclareMathSymbol{\sqleq}{\mathrel}{MnSyD}{90}
\DeclareMathSymbol{\sqgeq}{\mathrel}{MnSyD}{91}
\DeclareMathSymbol{\lessdot}{\mathrel}{MnSyD}{114}
\DeclareMathSymbol{\greaterdot}{\mathrel}{MnSyD}{115}
\DeclareMathSymbol{\leqslantdot}{\mathrel}{MnSyD}{118}
\DeclareMathSymbol{\geqslantdot}{\mathrel}{MnSyD}{119}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\nsqleq}{\mathrel}{MnSyD}{210}
\DeclareMathSymbol{\nsqgeq}{\mathrel}{MnSyD}{211}


==> tex-common/MnSymbol-medsquare.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\medsquare}{\mathord}{MnSyC}{106}


==> tex-common/MnSymbol-powerset.tex <==
% Bring in \powerset from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolpowerset}{\mathord}{MnSyC}{180}


==> tex-common/MnSymbol-triangles.tex <==
% Various triangles from MnSymbol. See http://tex.stackexchange.com/questions/36006.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\smalltriangleright}{\mathord}{MnSyC}{72}
\DeclareMathSymbol{\smalltriangleup}{\mathord}{MnSyC}{73}
\DeclareMathSymbol{\smalltriangleleft}{\mathord}{MnSyC}{74}
\DeclareMathSymbol{\smalltriangledown}{\mathord}{MnSyC}{75}
\DeclareMathSymbol{\filledtriangleright}{\mathord}{MnSyC}{76}
\DeclareMathSymbol{\filledtriangleup}{\mathord}{MnSyC}{77}
\DeclareMathSymbol{\filledtriangleleft}{\mathord}{MnSyC}{78}
\DeclareMathSymbol{\filledtriangledown}{\mathord}{MnSyC}{79}


==> tex-common/MnSymbol-twoheadarrows.tex <==
\DeclareFontFamily{U}{MnSymbolB}{}
\DeclareFontShape{U}{MnSymbolB}{m}{n}{
    <-6>  MnSymbolB5
   <6-7>  MnSymbolB6
   <7-8>  MnSymbolB7
   <8-9>  MnSymbolB8
   <9-10> MnSymbolB9
  <10-12> MnSymbolB10
  <12->   MnSymbolB12}{}
\DeclareFontShape{U}{MnSymbolB}{b}{n}{
    <-6>  MnSymbolB-Bold5
   <6-7>  MnSymbolB-Bold6
   <7-8>  MnSymbolB-Bold7
   <8-9>  MnSymbolB-Bold8
   <9-10> MnSymbolB-Bold9
  <10-12> MnSymbolB-Bold10
  <12->   MnSymbolB-Bold12}{}
\DeclareSymbolFont{MnSyB}{U}{MnSymbolB}{m}{n}

\DeclareFontFamily{U}{MnSymbolA}{}
\DeclareFontShape{U}{MnSymbolA}{m}{n}{
    <-6>  MnSymbolA5
   <6-7>  MnSymbolA6
   <7-8>  MnSymbolA7
   <8-9>  MnSymbolA8
   <9-10> MnSymbolA9
  <10-12> MnSymbolA10
  <12->   MnSymbolA12}{}
\DeclareFontShape{U}{MnSymbolA}{b}{n}{
    <-6>  MnSymbolA-Aold5
   <6-7>  MnSymbolA-Aold6
   <7-8>  MnSymbolA-Aold7
   <8-9>  MnSymbolA-Aold8
   <9-10> MnSymbolA-Aold9
  <10-12> MnSymbolA-Aold10
  <12->   MnSymbolA-Aold12}{}
\DeclareSymbolFont{MnSyA}{U}{MnSymbolA}{m}{n}

\let\twoheaddownarrow\relax
\DeclareMathSymbol{\twoheaddownarrow}{\mathrel}{MnSyA}{27}
\let\twoheaduparrow\relax
\DeclareMathSymbol{\twoheaduparrow}{\mathrel}{MnSyA}{25}

\let\ntwoheaddownarrow\relax
\DeclareMathSymbol{\ntwoheaddownarrow}{\mathrel}{MnSyB}{27}
\let\ntwoheaduparrow\relax
\DeclareMathSymbol{\ntwoheaduparrow}{\mathrel}{MnSyB}{25}


==> tex-common/MnSymbol-vdots.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolvdots}{\mathord}{MnSyC}{6}


==> tex-common/bigcdot.tex <==
% http://tex.stackexchange.com/questions/235118
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.7}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


==> tex-common/column-types.tex <==
% See http://tex.stackexchange.com/questions/12703/
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash\hspace{0pt}}p{#1}}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}


==> tex-common/curvetie.tex <==
% https://tex.stackexchange.com/questions/371292
% other solution based on halloweenmath, which is no longer in my TeX distribution...

\RequirePackage{pict2e}

\makeatletter
\DeclareRobustCommand{\curvetie}{\mathbin{\mathpalette\arc@bow@tie\relax}}
\newcommand{\arc@bow@tie}[2]{%
  \vcenter{\hbox{%
    \sbox\z@{$\m@th#1\otimes$}%
    \sbox\tw@{$\m@th\mkern1mu$}%
    \setlength{\unitlength}{\wd\z@}%
    \linethickness{.4\wd\tw@}%
    \begin{picture}(1,1)
    \polyline(0.7878,0.7878)(0.2122,0.2122)
    \polyline(0.2122,0.7878)(0.7878,0.2122)
    \put(0.5,0.5){\arc[-46,46]{0.4}}
    \put(0.5,0.5){\arc[134,226]{0.4}}
    \end{picture}%
  }}%
}
\makeatother


==> tex-common/line-shift.tex <==
% shift left, shift right line styles.

\usetikzlibrary{decorations}
\pgfdeclaredecoration{simple line}{initial}{
  \state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfmoveto{\pgfpointorigin}}
  \state{final}{\pgflineto{\pgfpointorigin}}
}
\tikzset{
   shift left/.style={decorate,decoration={simple line,raise=#1}},
   shift right/.style={decorate,decoration={simple line,raise=-1*#1}},
}


==> tex-common/localref.tex <==
% http://tex.stackexchange.com/questions/73112
\newcommand*{\proofContext}[1]{\def\currentprefix{proof:#1}}
\newcommand*{\locallabel}[1]{\label{\currentprefix:#1}}
\newcommand*{\localref}[1]{\ref{\currentprefix:#1}}
\newcommand*{\localeqref}[1]{\eqref{\currentprefix:#1}}


==> tex-common/mathabx-barharpoons.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\leftbarharpoon}        {3}{mathb}{"DC}
\DeclareMathSymbol{\rightbarharpoon}       {3}{mathb}{"DD}
\DeclareMathSymbol{\barleftharpoon}        {3}{mathb}{"DE}
\DeclareMathSymbol{\barrightharpoon}       {3}{mathb}{"DF}


==> tex-common/mathabx-bigoslash.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigoslash}{1}{mathx}{"CD}


==> tex-common/mathabx-bigotimes.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigotimes}{1}{mathx}{"C2}


==> tex-common/mathabx-primes.tex <==
% Setup the matha font (from mathabx.sty) -- because mathabx.sty incompatible with
% amsmath package.
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}

% Define some characters from mathabx.dcl.
\DeclareMathSymbol{\twoPrime}{3}{matha}{"32}
\DeclareMathSymbol{\threePrime}{3}{matha}{"33}
\DeclareMathSymbol{\fourPrime}{3}{matha}{"34}


==> tex-common/mathabx-sqbullet.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\sqbullet}{1}{mathb}{"0D}


==> tex-common/mathabx-wideparen.tex <==
% https://tex.stackexchange.com/questions/69323

%% code from mathabx.sty and mathabx.dcl
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\DeclareMathAccent{\wideparen}{0}{mathx}{"75}


==> tex-common/proof-helpers.tex <==
\RequirePackage{adjustbox}

% http://tex.stackexchange.com/questions/44933
\newcounter{myequation}
\makeatletter
\@addtoreset{equation}{myequation}
\makeatother

% http://tex.stackexchange.com/questions/82535
\newenvironment{proofalign}{\par\nobreak\small\noindent\flalign}{\endflalign}

\newcommand*{\proseDescription}{\paragraph{Prose description.}}
\newcommand*{\paragraphCase}[1]{\paragraph{\uline{#1}}}

\newcommand*{\absurd}[1]{\Absurd{\uline{#1}}}
\newcommand*{\Absurd}[1]{\textcolor{red}{#1}}
\newcommand*{\contradiction}{\Absurd{\bot}}
\newcommand*{\qedLocal}{\text{\ding{234}}\;}

\setlength{\ULdepth}{0.25em}
\newcommand*{\interCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseOne}[1]{%
& \indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseTwo}[1]{%
& \indent\indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSix}[1]{%
& \indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSeven}[1]{%
& \indent\indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}

\newcommand*{\introCaseDerivationZero}[2]{%
& \textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}

\newcommand*{\introCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.\;%
}

\newcommand*{\introSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}

% define \derivationWidth as a proportion of textwidth

\newcommand*{\caseDerivation}[2]{%
\textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}
\newcommand*{\derivation}[2]{%
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}


==> tex-common/relational-override.tex <==
% http://tex.stackexchange.com/questions/360021
\makeatletter
\DeclareRobustCommand{\reloverrideleft}{\mathrel{\mathpalette\rel@override\vartriangleleft}}
\DeclareRobustCommand{\reloverrideright}{\mathrel{\mathpalette\rel@override\vartriangleright}}

\newcommand{\rel@override}[2]{%
  \vphantom{#2}%
  \ooalign{$\m@th#1-$\cr$\m@th#1#2$}%
}
\makeatother


==> tex-common/secbreak.tex <==
\RequirePackage{fdsymbol}

\newcommand*{\secbreakchar}{\smblklozenge}
\newcommand*{\secbreak}{
\begin{center}%
   $\secbreakchar\;\secbreakchar\;\secbreakchar$%
\end{center}%
}


==> tex-common/theorem-envs.tex <==
% Not needed for llncs.sty or acmart.cls.
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{definition}{Definition}[subsection]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

% http://tex.stackexchange.com/questions/43966
\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother


==> tex-common/wavey.tex <==
% http://tex.stackexchange.com/questions/80378. This looks great, but unfortunately doesn't
% work properly with the Listings package; need to come up with an MWE and post a question.
\usepackage{xparse}
\usepackage{marginnote}
\usepackage{soul}
\usepackage{lipsum}
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\newlength\LineWidth
\newlength\Amplitude
\newlength\SegLength

\setlength\LineWidth{0.4pt}
\setlength\Amplitude{1pt}
\setlength\SegLength{5pt}

\definecolor{HLcolor}{RGB}{240,0,0}

% The following code contains a variation of the great code by Antal S-Z
% in his answer to http://tex.stackexchange.com/a/6029/3954
%in TeX.SX

\newcommand\tikzmark[1]{%
  \tikz[overlay,remember picture] \node (#1) {};}

\makeatletter
\newcommand{\highlight@DoHighlight}{
  \draw[HLcolor,line width=\LineWidth,decorate,decoration={zigzag,amplitude=\Amplitude,segment length=\SegLength}]  ($(begin highlight)+(0,-2pt)$) -- ($(end highlight)+(0,-2pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}
\makeatother

\DeclareDocumentCommand\Wavey{O{red}O{1pt}O{5pt}m}{%
  \colorlet{HLcolor}{#1}
  \setlength\Amplitude{#2}%
  \setlength\SegLength{#3}%
  \tikzmark{endquote}\tikzmark{beginquote}\highlight{#4}%
}


==> tex-common/xspace-emdash-fix.tex <==
% https://tex.stackexchange.com/questions/263271
\xspaceremoveexception{-}
\makeatletter
\renewcommand*\@xspace@hook{%
\ifx\@let@token-%
\expandafter\@xspace@dash@i
\fi
}
\def\@xspace@dash@i-{\futurelet\@let@token\@xspace@dash@ii}
\def\@xspace@dash@ii{%
\ifx\@let@token-%
\else
\unskip
\fi
-%
}
\makeatother

